Quantum stabilizer codes and beyond

The importance of quantum error correction in paving the way to build a practical quantum computer is no longer in doubt. This dissertation makes a threefold contribution to the mathematical theory of quantum error-correcting codes. Firstly, it extends the framework of an important class of quantum codes -- nonbinary stabilizer codes. It clarifies the connections of stabilizer codes to classical codes over quadratic extension fields, provides many new constructions of quantum codes, and develops further the theory of optimal quantum codes and punctured quantum codes. Secondly, it contributes to the theory of operator quantum error correcting codes also called as subsystem codes. These codes are expected to have efficient error recovery schemes than stabilizer codes. This dissertation develops a framework for study and analysis of subsystem codes using character theoretic methods. In particular, this work establishes a close link between subsystem codes and classical codes showing that the subsystem codes can be constructed from arbitrary classical codes. Thirdly, it seeks to exploit the knowledge of noise to design efficient quantum codes and considers more realistic channels than the commonly studied depolarizing channel. It gives systematic constructions of asymmetric quantum stabilizer codes that exploit the asymmetry of errors in certain quantum channels.

==> append.tex <==
\appendix{Title of Appendix}
This is the text of the Appendix. If this is the first appendix, it will be 
labelled Appendix A.


==> biblio.tex <==
\bibliographystyle{IEEEtranS}
\bibliography{codes,klappenecker,newrefs}


==> chAqecc.tex <==
\nix{
\usepackage{amsmath,paralist,amsthm,comment,amssymb}
\usepackage{times,color}
\usepackage{euler}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{ifthen}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\swt}{swt}
\DeclareMathOperator{\wt}{wt}

\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Hi}{\mathcal{H}}
\newcommand{\X}{{X}}
\newcommand{\Y}{{Y}}
\newcommand{\Z}{{Z}}
\newcommand{\sdual}{{\perp_s}}
\newcommand{\adual}{{\perp_a}}
\newcommand{\hdual}{{\perp_h}}
\newcommand{\one}{\mathbf{1}}

\newcommand{\R}{\mathcal{R}}
\newcommand{\bch}{\mathcal{BCH}}
\newcommand{\eg}{{\rm {EG}}}
\newcommand{\pg}{{\rm {PG}}}
\newcommand{\Rm}{{\rm {GRM}}}
\newcommand{\onemat}[0]{{\mathbf 1}}

\newcommand{\floor}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\nix}[1]{}
\newcommand{\mypar}[1]{{\bf #1.}}

%\newcommand{\ol}{\overline}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ds}{\displaystyle}
\newcommand{\scal}[2]{\langle #1\mid #2\rangle_s}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
}


%\begin{abstract}
  Recently, quantum error-correcting codes were proposed that
  capitalize on the fact that many physical error models lead to a
  significant asymmetry between the probabilities for bit flip and
  phase flip errors. An example for a channel which exhibits such
  asymmetry is the combined amplitude damping and dephasing channel,
  where the probabilities of bit flips and phase flips can be related
  to relaxation and dephasing time, respectively. We study asymmetric
  quantum codes that are obtained from the CSS construction. For such
  codes we derive upper bounds on the code parameters using linear
  programming. A central result of this paper is the explicit
  construction of some new families of asymmetric quantum stabilizer
  codes from pairs of nested classical codes and discuss their
  performance. We show that asymmetric quantum codes offer two
  advantages, namely to allow a higher rate without sacrificing
  performance when compared to symmetric codes and vice versa to allow
  a higher performance when compared to symmetric codes of comparable
  rates.  Our approach is based on a CSS construction that combines
  BCH and finite geometry LDPC codes.
%\end{abstract}


%\section{Introduction}

In many quantum mechanical systems the mechanisms for the occurrence
of bit flip and phase flip errors are quite different. In a recent
paper Ioffe and M\'{e}zard \cite{ioffe07} postulated that quantum
error-correction should take into account this asymmetry. The main
argument given in \cite{ioffe07} is that most of the known quantum
computing devices have relaxation times ($T_1$) that are around
$1{-}2$ orders of magnitude larger than the corresponding dephasing
times $(T_2)$. In general, relaxation leads to both bit flip and phase
flip errors, whereas dephasing only leads to phase flip errors.  This
large asymmetry between $T_1$ and $T_2$ suggests that bit flip errors
occur less frequently than phase flip errors and a well designed
quantum code would exploit this asymmetry of errors to provide better
performance.  In fact, this observation and its consequences for
xquantum error correction, especially quantum fault-tolerance, have
been studied in several papers \cite{aliferis07,evans07,stephens07}.

Our goal is to construct asymmetric quantum codes that exploit
asymmetry.  The focus in the present paper is on quantum memory and
communication, at present we do not consider the issue of fault
tolerance.  As a concrete illustration of this we
consider the amplitude damping and dephasing channel. For this channel
we can compute the probabilities of bit flip and phase flips in closed
form.  In particular, by giving explicit expressions for the ratio of
these probabilities in terms of the ratio $T_1/T_2$, we show how the
channel asymmetry arises.

\mypar{Related work} Several recent papers discuss the situation of
quantum error-correction in the presence of an asymmetric error model
that gives a strong bias towards certain errors.

In \cite{aliferis07} the authors give a construction based on
concatenation of repetition code with any other quantum code to get
asymmetric quantum codes for biased noise. While this has the
advantage that universal fault-tolerant quantum computation possible,
as shown in this paper, the codes constructed in this way have a lower
rate than the ones constructed in the present paper. On the other
hand, it is not known whether the codes presented in the present paper
admit a set of universal fault-tolerant gates that preserve the
channel asymmetry. The papers \cite{evans07,stephens07} use symmetric
CSS codes with asymmetric error correction strategy to obtain an
advantage for fault-tolerant quantum error correction over a symmetric
strategy. The asymmetry in this case comes from higher frequency of
syndrome measurements for the $X$-only generators as compared with the
$Z$-only generators.

The paper \cite{ioffe07} is closest to our work regarding the methods
used to construct asymmetric quantum codes as both \cite{ioffe07}
employ a CSS construction having a classical LDPC code for the
$Z$-errors and a classical BCH code for the $X$ errors. However, as we
show in Section \ref{sec:ldpcbch}, we employ a different approach to construct
the LDPC code which allows us to have more control on the degree
profile of the LDPC code. Arguably, this gives an advantage regarding
the structure of these codes on the one hand but also regarding their
performance since similar to the classical case, our codes do not show
an error floor for very small probabilities of channel errors.

It should also be noted that the performance of symmetric quantum
codes for some specific quantum codes, such as a $[[5,1,3]]$ or
$[[7,1,3]]$ codes, over arbitrary (not necessarily symmetric) Pauli
channels has been studied \cite{RDM:2002}. However, contrary to the
present paper in which the goal is to exploit channel asymmetries for
the code design, in this paper the goal is to merely characterize the
performance of a given code under variation of the error weights and
to find the channel under which the given code has optimal
performance. Finally, in a recent development \cite{FSW:2008} have
studied adaptive quantum error-correction strategies in which the
optimal error correction strategy is found for a given channel using
semidefinite programming. These techniques have been applied to the
case of asymmetric channels that arise from amplitude damping
channels, however, so far the adaptive methods have been applied to
symmetric quantum channels only.

\mypar{Organization of this paper} In Section \ref{sec:background} we
provide the necessary background on quantum channels and give a
motivation for asymmetric quantum channels, i.\,e., noise models which
show a significant bias toward specific types of errors. We consider
the concrete example of the noise model given by amplitude damping and
dephasing. This serves as motivation of asymmetric channels and has
the advantage that the amount of asymmetry in the bit flip in phase
flip probabilities can be quantified easily can be and related to
physical quantities such as $T_1$ and $T_2$.

Next, in Section \ref{sec:basics} we explain why our focus in this
paper will be asymmetric codes that are obtained from the
Calderbank-Shor-Steane (CSS) construction.  After briefly sketching
the ideas of asymmetric codes, we derive some bounds on the parameters
of these codes. Similar to the case of standard quantum codes, which
we will refer to symmetric quantum codes as they are not designed to
exploit any bias towards one specific error, it is possible to derive
good upper bounds using linear programming.

We then address the question of how to construct asymmetric quantum
codes.  In Section \ref{sec:constructions} we show that in general a
family of nested classical codes is well suited to constructing such
asymmetric quantum codes.  We illustrate this for a few well known
families of codes, namely Reed-Muller codes and BCH codes. Then we
propose an alternate approach to \cite{ioffe07} and use a finite
geometry LDPC code and BCH code to construct an asymmetric stabilizer
code.

The performance of asymmetric codes is subject of Section
\ref{sec:performance}. We simulate the performance of several examples
of asymmetric codes constructed by the methods described in this paper
in terms of the resulting block error rate versus the probability of
channel errors.  Simulations are carried out for various choices of
channel asymmetries and codes. We explain why a modification of the
standard iterative decoding algorithms known from classical LDPC codes
is required as in the quantum case no (soft) channel information is
available. We present a suitable modification of the iterative
decoding algorithm which starts with information in the check nodes
and then proceeds in a fashion similar to the classical hard decision
bit flipping algorithm.

\section{Background on quantum error models}
\label{sec:background}

Recall that a quantum channel is a completely positive trace
preserving map \cite{NC:2000}. Such maps can be written in Kraus
operator form where the action of the channel on a given input state
$\rho$ is described as follows: $\rho \mapsto \sum_i A_i \rho
A_i^\dagger$, where the completeness relation $\sum_i A_i^\dagger A_i=
\onemat$ holds. The operators $A_i$ are the Kraus operators of the
channel. A special case of a channel on one qubit arises if the Kraus
operators are simply given by the Pauli matrices, i.\,e., a state
$\rho$ is mapped to
\begin{eqnarray}\label{pauli-channel}
(1-p_x-p_y-p_z)\rho+ p_x\X\rho\X+p_y\Y\rho\Y + p_z\Z\rho\Z,
\end{eqnarray}
with 
\begin{eqnarray}
  \one= \left[\begin{smallmatrix} 1&0\\0&1\end{smallmatrix}\right];\quad
  \X= \left[\begin{smallmatrix} 0&1 \\1&0\end{smallmatrix}\right];	\quad
  \Y= \left[\begin{smallmatrix} 0&-i \\i&0\end{smallmatrix}\right];	\quad
  \Z= \left[\begin{smallmatrix} 1&0 \\0&-1\end{smallmatrix}\right].
	\label{eq:pauli}
\end{eqnarray}
Such a channel is called a \textit{Pauli channel}. In a Pauli channel
one has independent probabilities $p_x, p_y, p_z$ (subject to $p_x +
p_y +p_z \leq 1$) that an input qubit in state $\rho$ is subjected to a
Pauli $X$, $Y$, or $Z$ error, respectively.

As example of a channel that arises in the study decoherence in
concrete physical systems we consider the the combined
\textit{amplitude damping and dephasing channel} $\mathcal{E}$.
Important parameters for the noise process underlying this channel are
the relaxation time $T_1$ and dephasing time $T_2$. Suppose the
channel $\mathcal{E}$ acts on a single qubit state
$\rho=(\rho_{ij})_{i,j\in \{0,1\}}$ for a time $t$. This yields the
resulting density matrix
$$ \mathcal{E}(\rho) = 
\left[
\begin{array}{cc}
1-\rho_{11}e^{-t/T_1} & \rho_{01} e^{-t/T_2} \\
\rho_{10} e^{-t/T_2} 
& \rho_{11}e^{-t/T_1} 
\end{array}
\right]. 
$$  We would like to determine the probability
$p_x$, $p_y$, and $p_z$ such that an $X$, $Y$, or $Z$ error occurs in
a combined amplitude damping and dephasing channel. However, it turns
out that this question is not well-posed, since $\mathcal{E}$ is not a
Pauli channel, that is, it cannot be written in the form
(\ref{pauli-channel}). However, we can obtain a Pauli channel
$\mathcal{E}_T$ by conjugating the channel $\mathcal{E}$ by Pauli
matrices and averaging over the results. The channel $\mathcal{E}_T$
is called the Pauli-twirl of $\mathcal{E}$ and is explicitly given by

$$ \mathcal{E}_T(\rho) = \frac{1}{4} \sum_{A \in \{ \one, \X,\Y,\Z\}}
A^\dagger \mathcal{E}(A\rho A^\dagger )A.$$

Twirling \cite{DLT:2002,EAZ:2005,dankert06} is used in quantum
information theory as a tool to map quantum channels to simpler ones,
while preserving many interesting features of the initial channel.
Twirling has been used for instance for the task of estimating the
average fidelity of a quantum gate and for the task of determining
more general features of channels \cite{ESR+:2007} as well as for the
task of identifying codes for general quantum channels
\cite{SMKE:2007}. In our situation we apply Pauli to map the channel
$\mathcal{E}$ to a Pauli channel.

\begin{theorem}\label{th:amplitudedamping}
  Given a combined amplitude damping and dephasing channel
  $\mathcal{E}$ as above, the associated Pauli-twirled channel is of
  the form
$$\mathcal{E}_T(\rho) = (1-p_x-p_y-p_z)\rho+ p_x\X\rho\X+p_y\Y\rho\Y +
p_z\Z\rho\Z,$$
where $p_x=p_y=(1-e^{-t/T_1})/4$ and $p_z=1/2-p_x-\frac{1}{2}e^{-t/T_2}$. 
In particular,
$$ \frac{p_z}{p_x} =1+2 \frac{1-e^{t/T_1(1-T_1/T_2)}}{e^{t/T_1}-1}.
$$ 
If $t\ll T_1$, then we can approximate this ratio as $2T_1/T_2-1$.
\end{theorem}

The proof of this theorem is straightforward but technical and is
given in Appendix \ref{app:theorem1}. From Theorem
\ref{th:amplitudedamping} follows that an asymmetry in the $T_1$ and
$T_2$ times does translate to an asymmetry in the occurrence of bit
flip and phase flip errors.  Note that $p_x=p_y$ indicating that the
$\Y$ errors are as unlikely as the $\X$ errors.  We shall refer to the
ratio $p_z/p_x$ as the channel asymmetry and throughout the paper
shall denote it by $A$.

\section{Asymmetric quantum codes: basics and bounds}
\label{sec:basics}

Asymmetric codes use the fact the phase errors are much more likely
than the bit flip errors or the combined bit-phase flip errors.
Therefore the code has different error correcting capability for
handling different type of errors. We require the code to correct many
phase errors but it is not require to handle the same number of bit
flip errors. If we assume a CSS code, then we can meaningfully speak
of $X$-distance and $Z$-distance. A CSS stabilizer code as that can
detect all $X$ errors up to weight $d_x-1$ is said to have an
$X$-distance of $d_x$.  Similarly if it can detect all $Z$ errors up to
weight $d_z-1$, then it is said to have a $Z$-distance of $d_z$. We
shall denote such a code by $[[n,k,d_x/d_z]]_q$ to indicate it is an
asymmetric code.  We could also view this code as an $[[n,k,\min\{
d_x,d_z\}]]_q$ stabilizer code.  Further extension of these metrics to
an additive non-CSS code is an interesting problem, but we will not go
into the details here. Though the notion of asymmetric nonbinary
quantum codes needs further treatment, the idea of nonbinary CSS is
well understood. Some of the results are given for a nonbinary
alphabet.

We will exclusively use the CSS construction \cite{calderbank98} to
construct asymmetric quantum codes.  Recall that in the CSS
construction a pair of codes are used, one for correcting the bit flip
errors and the other for correcting the phase flip errors. Our choice
of these codes will be such that the code for correcting the phase
errors has a larger distance than the code for correcting the bit flip
errors. We restate the CSS construction in a form convenient for
asymmetric stabilizer codes.

\begin{lemma}[CSS Construction \cite{calderbank98}]\label{lm:css}
  Let $C_x, C_z$ be linear codes over $\F_q^n$ with the parameters
  $[n,k_x]_q$, and $[n,k_z]_q$ respectively. Let $C_x^\perp\subseteq
  C_z$.  Then there exists an $[[n,k_x+k_z-n,d_x/d_z]]_q$ asymmetric
  quantum code, where $d_x=\wt(C_x\setminus C_z^\perp)$ and
  $d_z=\wt(C_z\setminus C_x^\perp)$
\end{lemma}
If in the above construction $d_x=\wt(C_x)$ and $d_z=\wt(C_z)$, then
we say that the code is pure. In this context, we can give a bound for
CSS type pure asymmetric stabilizer codes similar to the quantum
Singleton bound.

\begin{lemma}\label{lm:cssBoundPure}
A pure asymmetric $[[n,k,d_x/d_z]]_q$ CSS code satisfies 
$$ k\leq n-d_x-d_z+2.$$
\end{lemma}
\begin{proof}
  Assume that the asymmetric code is constructed using
  Lemma~\ref{lm:css}, then $\wt(C_x)=d_x$ and $\wt(C_z)=d_z$. By the
  classical Singleton bound $|C_x|\leq q^{n-d_x+1}$ and $|C_z|\leq
  q^{n-d_z+1}$.  Then $|C_x|\cdot |C_z|= q^{n+k} \leq
  q^{2n-d_x-d_z+2}$. It follows $k\leq n-d_x-d_z+2$.
\end{proof}

The bound in Lemma~\ref{lm:cssBoundPure} can be extended for all
$\F_q$-linear asymmetric CSS type codes.
\begin{lemma}\label{lm:cssBoundImpure}
Any CSS type $\F_q$-linear $[[n,k,d_x/d_z]]_q$ CSS type code satisfies
\begin{eqnarray}
 k\leq n-d_x-d_z+2.\end{eqnarray}
\end{lemma}
\begin{proof}
  Let us assume that the asymmetric CSS code was constructed using
  Lemma~\ref{lm:css}.  Let $C^c_x$ be the complement of $C_z^\perp$ in
  $C_x$ {\em i.e.}, a subcode of $C_x$ such that span of $C_x^c$ and
  $C_z^\perp$ is $C_x$.  Similarly, let $C_z^c$ be the complement of
  $C_x^\perp$ in $C_z$.  Let $\dim C_x^\perp=k_a$ and $\dim C_z^\perp
  =k_b$. We have $|C_x^\perp|\cdot |C_z^\perp|=q^{n-k}=q^{k_a+k_b}$.
  Now the $\F_q$-linearity of the stabilizer code implies that we can
  choose $C_x^c$ to be all zeros in $k_b$ columns, because we can
  perform Gaussian elimination using $C_z^\perp$ to get rid of the
  nonzero elements in $k_b$ columns.  In effect $C_x^c$ is a code of
  length $n-k_b$.  Now the classical Singleton bound implies that
  $|C_x^c|\leq q^{(n-k_b)-d_x+1}$.  The minimum distance of $C_x^c$
  must be at least $d_x$ because it is a subcode of $C_x\setminus
  C_z^\perp$ and we know that $d_x=\wt(C_x\setminus C_z^\perp)$.
  Similarly we can show that $|C_z^c|\leq q^{(n-k_a)-d_z+1}$, where
  $d_z=\wt(C_z\setminus C_x^\perp)$.  It follows that
$$|C_x^c|\cdot |C_z^c| \leq q^{n-k_b-d_x+1} q^{n-k_a-d_z+1} = q^{2n-k_a-k_b-d_x-d_z+2}.$$
But $|C_x^\perp|\cdot |C_z^\perp|=q^{n-k}=q^{k_a+k_b}$, therefore
$$|C_x^c|\cdot |C_z^c| \leq q^{2n-k_a-k_b-d_x-d_z+2} = q^{n+k-d_x-d_z+2}.$$
Now using the fact that $|C_x^c|\cdot |C_z^c| =q^{2k}$, we have $
q^{k} \leq q^{n-d_x-d_z+2}$ {\em i.e.} $k\leq n-d_x-d_z+2$.
\end{proof}
This bound seems to imply that if there was an asymmetry in the
channel, then using asymmetric quantum codes we could potentially gain
in rate.  It would be interesting to extend this bound to all
asymmetric stabilizer codes linear or otherwise.  The (quantum)
Singleton bound in general is not very tight, especially for large
lengths.  In this context the linear programming bounds turn out to be
more useful. We shall derive some linear programming bounds for CSS
type asymmetric stabilizer codes.

\begin{theorem}[Linear programming bounds]\label{th:lp}
  If an $[[n,k,d_x/d_z]]_2$ asymmetric CSS stabilizer code with $k>0$
  exists, then there exists a solution to the optimization problem:
  maximize $\sum_{j=1}^{d_z-1} A_j$ subject to the constraints
\begin{enumerate}
\item $A_0=A_0^\perp=B_0=B_0^\perp=1$ and $A_j, A_j^\perp, B_j,
  B_j^\perp \geq 0$ for all $1\le j\le n$;
\item $0 < k'< n-k$
\item $\ds\sum_{j=0}^n A_j =2^{k'}$ 
\item  $\ds\sum_{j=0}^n B_j = 2^{n-k-k'}$;
\item $A_j^\perp = \ds\frac{1}{2^{k'}} \sum_{r=0}^n K_j(r)A_r$ for all
  $j$ in the range $0\le j \le n $;
\item $B_j^\perp = \ds\frac{1}{2^{n-k-k'}} \sum_{r=0}^n K_j(r)B_r$ for
  all $j$ in the range $0\le j \le n $;
\item $A_j=B_j^\perp$ for all $j$ in $0\le j<d_x$ and $A_j \leq
  B_j^\perp$ for all $d_x\le j\le n$;
\item $B_j=A_j^\perp$ for all $j$ in $0\le j<d_z$ and $B_j\leq
  A_j^\perp$ for all $d_z \le j\le n$;
\end{enumerate}
where the coefficients $A_j, A_j^\perp, B_j$ and $B_j^\perp$ are integral and
$K_j(r)$ denotes the Krawtchouk polynomial
\begin{eqnarray}
 K_j(r) = \sum_{s=0}^j (-1)^s \binom{r}{s}\binom{n-r}{j-s}.
\end{eqnarray}
\end{theorem}
\begin{proof}
  If an $[[n,k,d_x/d_z]]_2$ asymmetric stabilizer code exists, then by
  Lemma~\ref{lm:css} there exists classical codes $C_x^\perp \subseteq
  C_z\subseteq \F_2^{n}$.  Let the weight distributions of $C_z^\perp$
  and $C_x^\perp $ be given by $A_i,B_i$ respectively, where $0\leq
  i\leq n $.  If we let $|C_z^\perp|=2^{k'}$, then this means $\sum
  A_i =2^{k'}$ and since $|C_x^\perp|\cdot |C_z^\perp|=2^{n-k}$, it
  follows that $\sum B_i = 2^{n-k-k'}$. We restrict the range of
  $0<k'<n-k$ to ensure that $d_x,d_z>1$.  The weight distributions of
  $C_x$ and $C_z$ are given by the MacWilliams duality relations
  \cite{macwilliams77}. These give us
\begin{eqnarray}
A_j^\perp &= & \ds\frac{1}{2^{k'}} \sum_{r=0}^n K_j(r)A_r,\\	
	B_j^\perp & =& \ds\frac{1}{2^{n+k-k'}} \sum_{r=0}^n K_j(r)B_r.
\end{eqnarray}

Since $C_z^\perp \subseteq C_x$ and $C_x^\perp \subseteq C_z$ we must
have $A_j \leq B_j^\perp $ and $B_j \leq A_j^\perp$, for $0\leq j\leq
n$.  As the quantum code has $X$-distance $d_x$, all vectors of weight
less than $d_x$ in $C_x$ must be in $C_z^\perp$ giving us
$A_j=B_j^\perp$ for $1\leq j\leq d_x-1$. Similarly all vectors of
weight less than $d_z$ in $C_z $ must be in $C_x^\perp$ and we get
$B_j=A_j^\perp$, for $1\leq j\leq d_z-1$.
\end{proof}

In order to implement the above constraints as a linear programming
problem we must fix the value of $k'$. Then the above constraints
reduce to $n-k-1$ instances of a linear programming problem. An
$[[n,k,d_x/d_z]]$ code will not exist if none of the instances have a
solution. It is possible that the code might not exist even if some
instance has a solution.

Using the linear programming bounds we were able to show that there
can exist a $[[15,1,3/7]]$ code. This code can be constructed using
two BCH codes. Further details about this code are given in
Section~\ref{sec:performance}. Note that there does not exist a
$[[15,1,7]]$ stabilizer code.

A subtle point regarding the application of the linear programming
bounds should be kept in mind. The linear programming bounds indicate
that the smallest nontrivial asymmetric code encoding one qubit and
able to correct a single X error and at least two Z errors is of
length 12. The best possible distance that can be obtained with
parameters $[[12,1]]$ is 5. However it must be noted that no
$[[12,1,5]]$ CSS exists. This is a crucial difference because the
performance of the $[[12,1,5]]$ CSS and non-CSS codes is different. In
fact under bounded distance decoding the CSS code will have a lower
error rate than the non-CSS code, assuming it exists.  The LP bounds
also indicate that a $[[12,1,3/5]]$ CSS code may exist.  It would be
an interesting problem to show its existence or nonexistence. A small
code might be easier to study to gain insight into asymmetric quantum
error-correction.

\section{Asymmetric quantum codes: constructions}
\label{sec:constructions}

\subsection{Construction from families of nested codes}

Our first construction makes use of Reed-Muller codes (see
\cite[pg~33--36]{huffman03} for an introduction).  Recall that a
Reed-Muller code of order $r$ and length $2^m$ has the parameters
$[2^m,\sum_{j=0}^r \binom{m}{j},2^{m-r}]$. Let us denote an $r$th
order Reed-Muller code as $\R(r,m)$. Reed-Muller codes have the
following interesting properties of relevance for us.
\begin{compactenum}[i)]
\item $\R(r,m)^\perp=\R(m-1-r,m)$
\item $\R(r_1,m)\subseteq \R(r_2,m)$ if $r_1\leq r_2$
\end{compactenum}

\medskip We shall call a family of codes which satisfy a property like
ii) with respect to some code parameter \textsl{nested codes}. The BCH
codes are also a family of nested codes. As a first example we
construct asymmetric quantum codes based on the nested family of
Reed-Muller codes. The resulting codes are not new, they have been
already constructed in \cite{steane99b}.

\begin{lemma}[Asymmetric RM Stabilizer Codes]\label{lm:rmAqecc}
Let $0\leq r_1 < r_2 <m$. Then there exists an 
$$[[2^m,\sum_{j=r_1+1}^{r_2}\binom{m}{j}, 2^{m-r_2}/2^{r_1+1}]]_2$$
asymmetric RM stabilizer code.
\end{lemma}
\begin{proof}
  Let $ C_x = \R(r_2,m)$ and $ C_z = \R(m-1-r_1,m)=\R(r_1,m)^\perp$.
  Then the code follows from the application of Lemma~\ref{lm:css}.
  Note that the dimension of the quantum code is
$$k_x+k_z-n= k_x-\dim C_z^\perp = \sum_{j=0}^{r_2}\binom{m}{j} - 
\sum_{j=0}^{r_1}\binom{m}{j} =\sum_{j=r_1+1}^{r_2}\binom{m}{j},$$
where the last equality follows form the fact $r_1< r_2$.  With
respect to the distance, we have $d_x=\wt(C_x\setminus C_z^\perp) =
\wt(\R(r_2,m)\setminus\R(r_1,m)) =2^{m-r_2}$, because the
$\wt(\R(r_1,m))=2^{m-r_1}>2^{m-r_2}=\wt(\R(r_2,m))$.  Similarly,
$d_z=\wt(C_z\setminus C_x^\perp)=
\wt(\R(m-1-r_1,m)\setminus\R(m-1-r_2,m)) = 2^{r_1+1}$.
\end{proof}
These codes illustrate the trade offs involved in the design of
asymmetric stabilizer codes. In order to have large asymmetry in the
distance we need to have $d_x/d_z$ to be very small.  In this case we
need $2^{r_1+r_2+1-m}$ large. In order to get a large rate we will
require that the difference between $r_2-r_1$ also large.

\nix{
\begin{example}
Suppose we let $m=10$ and vary $r_1$ and $r_2$. Then we have the following
codes.
\begin{table}[htb]
\begin{center}
\begin{tabular}{c|c|c|c|c}
$r_1$&$r_2$  & Code &  Rate & Asymmetry \\
     &  & $[[n,k,d_x/d_z]]_2$ &  k/n &  $d_z/d_x$ \\\hline
%8&9  & $[[1024,10,2/512]]_2 $&   & 256 \\
%7&9  & $[[1024,55,2/256]]_2 $&   & 128 \\
%6&9  & $[[1024,175,2/128]]_2 $&   & 64 \\
%5&9  & $[[1024,385,2/64]]_2 $&   & 32 \\\hline
7&8  & $[[1024,45,4/256]]_2 $&   & 64 \\
6&8  & $[[1024,165,4/128]]_2 $&   & 32 \\
5&8  & $[[1024,375,4/64]]_2 $&   & 32 \\\hline
6&7  & $[[1024,120,8/128]]_2 $&   & 16 
\end{tabular}
\end{center}
\caption{Asymmetric RM stabilizer codes}
\label{tab:rmAqecc}
\end{table}
\end{example}
}

\begin{lemma}[Rate gain for RM AQECC]
Let $0\leq \Delta r\leq r\leq \floor{(m-1)/2}$, then there exists an
$[[2^m,\sum_{j=r+1}^{m-1-r}\binom{m}{j},2^{r+1}]]_2$ code which can be 
turned into an 
$$[[2^m,\sum_{j=r+1}^{m-1-r}\binom{m}{j}+\Delta k,2^{r+1-\Delta r}/2^{r+1}]]_2$$
asymmetric code where
$$\Delta k=\sum _{m-r}^{m-1-r+\Delta r}\binom{m}{j}.$$
\end{lemma}
\begin{proof}
Under the conditions on $r$, we can choose $C_x=C_z=\R(m-1-r,m)$ and apply
Lemma~\ref{lm:css}, then the stabilizer code follows. If we choose
$C_x=\R(m-1-r+\Delta r,m)$, then we can convert the stabilizer code into
the asymmetric stabilizer code with the given parameters.  
\end{proof}

The preceding result indicates that asymmetry can be exploited
to get higher rates compared to a symmetric stabilizer code. 

\begin{example} 
  \rm In Table~\ref{tab:rmqecc} we show the gains in rate as one
  allows for more and more asymmetry.
\begin{table}[htb]
\begin{center}
\begin{tabular}{c|c|c|c|c}
$r$  & Symmetric & \multicolumn{3}{c}{Asymmetric  code} \\
     & code $[[n,k,d]]_2$ & \multicolumn{3}{c}{$[[n,k,d_x/d_z]]_2$} \\\hline
 $\Delta r$   & 0   &1 &2&3 \\\hline
4& $[[1024,252,32]]_2 $&  $[[1024,462,16/32]]_2$&$[[1024,582,8/32]]_2$&$[[1024,627,4/32]]_2$ \\
3& $[[1024,672,16]]_2 $&  $[[1024,792,8/16]]_2$&$[[1024,837,4/16]]_2$ 
&$[[1024,847,2/16]]_2$\\
2& $[[1024,912,8]]_2  $&  $[[1024,957,4/8]]_2$&$[[1024,967,2/8]]_2  $\\
1& $[[1024,1002,4]]_2 $& $[[1024,1012,2/4]]_2 $&\\
\end{tabular}
\end{center}
\caption{Asymmetric quantum codes constructed from the nested codes
construction applied to Reed-Muller stabilizer codes.}
\label{tab:rmqecc}
\end{table}
\end{example}

Denote a binary narrow-sense primitive BCH code of length $n=2^m-1$
and design distance $\delta=2t+1$ as $\bch(\delta)$. If $\delta \leq
2^{\ceil{m/2}}-1$, we can compute the dimension of the BCH code
exactly as $2^m-1- mt$, see
\cite[Corollary~8]{macwilliams77}\footnote{Actually, this relation
  holds for $\delta\leq 2^{\ceil{m/2}}+3$. But this suffices for our
  purposes.}. In the following we assume that the design distances of
binary BCH codes are odd.

\begin{lemma}[Asymmetric BCH Stabilizer Codes]\label{lm:bchAqecc}
  Let $m\geq 2$ and $2\leq \delta_1 < \delta_2 <\delta_{\max}$, where
  $\delta_{\max}=2^{\ceil{m/2}}-1$ and $\delta_i\equiv 1\bmod 2$. Then
  there exists an
$$[[2^m-1,m(\delta_2-\delta_1)/2, d_x/d_z ]]_2$$
asymmetric BCH stabilizer code, where $d_x\geq \delta_1$ and $d_z \geq
\delta_{\max}+1$.
\end{lemma}
\begin{proof}
  In this case we choose $C_x= \bch(\delta_1)$ and
  $C_y=\bch(\delta_2)^\perp$. Under the restrictions on $\delta_1$ and
  $\delta_2$, we can compute the dimension of the BCH codes
  explicitly.  The dimension of $\bch(\delta)^\perp$ is given by
  $m(\delta-1)/2$, assuming odd $\delta$. By Lemma~\ref{lm:css} we can
  then compute the dimension of the quantum code as $m(\delta_2-1)/2-
  m(\delta_1-1)/2 = m(\delta_2-\delta_1)/2$.

  We have $d_x\geq \wt(\bch(\delta_1)\setminus \bch(\delta_2)) \geq
  \delta_1$ and $d_z\geq \wt(\bch(\delta_2)^\perp\setminus
  \bch(\delta_1)^\perp) \geq \delta_{\max}$. The last inequality
  follows from the fact that the distance of $\bch(\delta_2)^\perp$
  code is at least $\delta_{\max}+1$ as shown in
  \cite[Lemma~10]{aly07}.
\end{proof}

\begin{example}
  \rm Suppose we let $m=10$ and vary $\delta_1$ and $\delta_2$. Some
  of the codes that can be constructed are given in
  Table~\ref{tab:bchAqecc}.
\begin{table}[htb]
\begin{center}
\begin{tabular}{c|c|c|c|c}
$\delta_1$&$\delta_2$  & Code &  Rate & Asymmetry \\
     &  & $[[n,k,d_x/d_z]]_2$ &  k/n &  $d_z/d_x$ \\\hline
29&31  & $[[1023,10,29/32]]_2 $&   0.00978&  $\approx 1$\\
%27&31  & $[[1023,20,27/32]]_2 $&   &  \\
%25&31  & $[[1023,30,25/32]]_2 $&   &  \\
%23&31  & $[[1023,40,23/32]]_2 $&   &  \\
%21&31  & $[[1023,50,21/32]]_2 $&   &  \\
%19&31  & $[[1023,60,19/32]]_2 $&   &  \\
17&31  & $[[1023,70,17/32]]_2 $&   0.06843&  \\
15&31  & $[[1023,80,15/32]]_2 $&   0.07820& $\approx2$ \\
13&31  & $[[1023,90,13/32]]_2 $&  0.08798 &  \\
11&31  & $[[1023,100,11/32]]_2 $&  0.09775 & $\approx3$ \\
9&31  & $[[1023,110,9/32]]_2 $&   0.10753&  \\
7&31  & $[[1023,120,7/32]]_2 $&  0.11730 & $\approx4$ \\
5&31  & $[[1023,130,5/32]]_2 $&  0.12708 & $\approx6$ \\
3&31  & $[[1023,140,3/32]]_2 $&  0.13685 &  $\approx10$\\\hline
27&29  & $[[1023,10,27/32]]_2 $&  0.00978 &  $\approx 1$\\
15&29  & $[[1023,60,15/32]]_2 $&   0.05865&  $\approx 2$\\
9&29  & $[[1023,100,9/32]]_2 $&  0.09775 &  $\approx 3$\\
7&29  & $[[1023,110,7/32]]_2 $&   0.10753 &  $\approx 4$\\
5&29  & $[[1023,120,5/32]]_2 $&  0.11730   &  $\approx 6$\\
3&29  & $[[1023,130,3/32]]_2 $&  0.12708   &  $\approx 10$\\
\end{tabular}
\end{center}
\caption{Asymmetric quantum codes constructed from the nested codes
construction applied to BCH stabilizer codes.}
\label{tab:bchAqecc}
\end{table}
\end{example}

Alternatively, we could consider dual containing BCH codes to
construct stabilizer codes. In this case it is easier to see that the
gain in rate is proportional to the loss in the distance for the bit
flip channel.

\begin{lemma}
  Let $n=2^m-1$, $\delta_{\max}=2^{\ceil{m/2}}-1$ and $\delta=2t+1\leq
  \delta_{\max}$.  Then there exists an $[[n,n-m(\delta-1),\geq \delta
  ]]_2$ stabilizer code that can be converted to an
  $[[n,n-m(\delta-1)+m\Delta/2,d_x/d_z]]_2$ asymmetric stabilizer code
  where $0\leq \Delta=2l\leq \delta-2$ and $d_x\geq \delta-\Delta$ and
  $d_z\geq \delta$.
\end{lemma}
\begin{proof}
  Under the restrictions on $\delta$, we have $\bch(\delta)^\perp
  \subseteq \bch(\delta)$, see \cite[Lemma~1]{steane99}. Then the
  stabilizer code is obtained by choosing $C_x=C_z=\bch(\delta)$ in
  Lemma~\ref{lm:css}.  If $C_x$ is chosen to be $\bch(\delta
  -\Delta)$, then we get the asymmetric stabilizer code.
\end{proof}
These results seem to indicate the once again that asymmetry in
general can lead to a rate gain. In the case of the BCH stabilizer
codes constructed above it appears that the rate gain is linearly
proportional to the reduction in the distance of the code used for
correcting bit flip errors.

In general any family of nested codes can lead to a class of
asymmetric stabilizer codes. The main obstacle to such a method is
usually the knowledge of the dual distances, a knowledge of which is
required to determine the error correcting capability of the quantum
code. However, algebraic codes have this nice structure of being
nested and within certain ranges it is also possible to lower bound
the distances including the dual distances. So while we cannot claim a
truly asymmetric code because of our lack knowledge of these distances
we can certainly form a class of codes quite suitable for the
asymmetric channels.

\subsection{Construction from dual pairs of LDPC and BCH codes}
\label{sec:ldpcbch}

Nested codes are not the only method to construct asymmetric codes.
Ioffe and M\'{e}zard used a combination of BCH and LDPC codes to
construct asymmetric codes. The intuition being that the stronger LDPC
code should be used for correcting the phase errors and the BCH code
can be used for the infrequent bit flips. This essentially reduces to
finding a good LDPC code such that the dual of the LDPC code is
contained in the BCH code. They solve this problem by randomly
choosing codewords in the BCH code which are of low weight (so that
they can be used for the parity check matrix of the LDPC code).
However, their method is a little ad hoc and it is not clear how good
is the resulting LDPC code.  For instance, the degree profiles of the
resulting code are regular and there is little control over the final
degree profiles of the code.  It was claimed in \cite{ioffe07} that
their codes can be analyzed using the traditional methods of analysis
for the LDPC codes. But there are many questions that must be answered
before it can be fully be justified. For instance, it is not apparent
what ensemble or degree profiles one will use for performing this
analysis.

We consider using LDPC codes to construct asymmetric stabilizer codes.
Part of the reason being that these codes are among the best classical
codes with efficient decoding algorithms. It should be noted that
several classes of quantum LDPC codes have been proposed
\cite{mackay04,camara05,hagiwara07}. So far, however, the structure of
quantum LDPC codes in general, including their decoding algorithms, is
not well understood. For some time it was even doubtful whether
quantum LDPC codes exist at all, since a simple observation shows for
instance that quantum LDPC codes constructed as stabilizer codes must
necessarily have $4$-cycles in their Tanner graph. To circumvent this
problem, we are interested in families of quantum LDPC codes which
have the property to tolerate large numbers of $4$-cycles without
affecting the performance of the decoding algorithm too adversely.

More precisely, we propose two families of quantum codes based on LDPC
codes.  In the first case we use LDPC codes for both the $X$ and $Z$
channel. We will need the following facts about generalized
Reed-Muller codes and finite geometry LDPC codes.

\subsubsection{Some facts about finite geometry LDPC codes
  \cite{kou01,tang05}}
Let us denote by $\eg(m,p^s)$ the Euclidean finite geometry over
$\F_{p^s}$ consisting of $p^{ms}$ points. For our purposes it only
suffices to use the fact that this geometry is equivalent to the
vector space $\F_{p^s}^m$.  A $\mu$-dimensional subspace of
$\F_{p^s}^m$ or its coset is called a \textsl{$\mu$-flat}. Assume that
$0\leq \mu_1< \mu_2\leq m$.  Then we denote by
$N_{\eg}(\mu_2,\mu_1,s,p)$ the number of $\mu_1$-flats in a
$\mu_2$-flat and the $A_{\eg}(m,\mu_2,\mu_1, s,p)$, the number of
$\mu_2$-flats that contain a given $\mu_1$-flat. These are given by
(see \cite{tang05})
\begin{eqnarray}
N_{\eg}(\mu_2,\mu_1,s,p)&=& q^{(\mu_2-\mu_1)}\prod_{i=1}^{\mu_1}
\frac{q^{\mu_2-i+1}-1}{q^{\mu_1-i+1}-1};\label{eq:nEG}\\
A_{\eg}(m,\mu_2,\mu_1,s,p)&=& \prod_{i=\mu_1+1}^{\mu_2}
\frac{q^{m-i+1}-1}{q^{\mu_2-i+1}-1}, \label{eq:aEG}
\end{eqnarray}
where $q=p^s$.  Index all the $\mu_1$-flats from $i=1$ to
$n=N_{\eg}(m,\mu_1,s,p)$ as $F_i$.  Let $F$ be a $\mu_2$-flat in
$\eg(m,p^s)$.  Then we can associate an incidence vector to $F$ with
respect to the $\mu_1$ flats as follows.
$$
\mathfrak{i}_F = \left\{i_j\mid \begin{array}{cl}i_j =1 &\mbox{ if $F_j$ is contained in } F \\
i_j=0& \text{otherwise.}\end{array}
\right\}.
$$
Index the $\mu_2$-flats from $j=1$ to $J=N_{\eg}(m,\mu_2,s,p)$.
Construct the $J\times n $ matrix $H_{\eg}^{(1)}(m,\mu_2,\mu_1,s,p)$
whose rows are the incidence vectors of all the $\mu_2$-flats with
respect to the $\mu_1$-flats. This matrix is also referred to as the
incidence matrix.  Then the type-I Euclidean geometry code from
$\mu_2$-flats and $\mu_1$-flats is defined to be the null space of the
$\F_p$-linear span of $H_{\eg}^{(1)}(m,\mu_2,\mu_1,s,p)$. This is
denoted as $C_{\eg}^{(1)}(m,\mu_2,\mu_1,s,p)$.  Let
$H_{\eg}^{(2)}(m,\mu_2,\mu_1,s,p) =
H_{\eg}^{(1)}(m,\mu_2,\mu_1,s,p)^t.$ Then the type-II Euclidean
geometry code $C_{\eg}^{(2)}(m,\mu_2,\mu_1,s,p)$ is defined to be the
null space of $H_{\eg}^{(2)}(m,\mu_2,\mu_1,s,p)$. Let us now consider
the $\mu_2$-flats and $\mu_1$-flats that do not contain the origin of
$\eg(m,p^s)$. Now form the incidence matrix of the $\mu_2$-flats with
respect to the $\mu_1$-flats not containing the origin.  The null
space of this incidence matrix gives us a quasi-cyclic code in
general, which we denote by $C_{\eg,c}^{(1)}(m,\mu_2,\mu_1,s,p)$.

\subsubsection{Some fact about generalized Reed-Muller codes
  \cite{kasami68}} Let $\alpha$ be a primitive element in
$\F_{q^{m}}$.  The cyclic generalized Reed-Muller code of length
$q^m-1$ and order $\nu$ is defined as the cyclic code with the
generator polynomial whose roots $\alpha^j$ satisfy $0<j\leq
m(q-1)-\nu-1$. The generalized Reed-Muller code is the singly extended
code of length $q^m$.  It is denoted as $\Rm_q(\nu,m)$. The dual of a
GRM code is also a GRM code \cite{assmus98,blahut03,kasami68}.  It is
known that
\begin{eqnarray}
\Rm_q(\nu,m)^\perp = \Rm_q(\nu^\perp,m) \quad \text{with}
\quad \nu^\perp = m(q-1)-1-\nu.
\end{eqnarray}

Let $C$ be a linear code over $\F_{q^s}^n$. Then we define
$C|_{\F_q}$, the \textsl{subfield subcode} of $C$ over $\F_q^n$ as the
codewords of $C$ which are entirely in $\F_q^n$, (see
\cite[pages~116-120]{huffman03}). Formally this can be expressed as
\begin{eqnarray}
C|_{\F_q} = \{c\in C\mid c\in \F_q^n \}.
 \end{eqnarray}
 Let $C\subseteq \F_{q^l}^n$. The the \textsl{trace code} of $C$ over
 $\F_q$ is defined as
\begin{eqnarray}
\tr_{q^l/q}(C) = \{\tr_{q^l/q}(c) \mid c\in C\}.
\end{eqnarray}
There are interesting relations between the trace code and the
subfield subcode. One of which is the following result which we will
need later.
\begin{lemma}\label{lm:inclusion}
Let $C\subseteq \F_{q^l}^n$. Then $C|_{\F_q}$, the subfield subcode of $C$
is contained in $\tr_{q^l/q}(C)$, the trace code of $C$. In other words
$$ C|_{\F_q}\subseteq \tr_{q^l/q}(C).$$
\end{lemma}
\begin{proof}
  Let $c\in C|_{\F_q} \subseteq \F_q^n$ and $\alpha \in \F_{q^l}$.
  Then $\tr_{q^l/q}(\alpha c)= c\tr_{q^l/q}(\alpha)$ as $c\in \F_q^n$.
  Since trace is a surjective form, there exists some $\alpha\in
  \F_{q^l}$, such that $\tr_{q^l/q}(\alpha)=1$. This implies that
  $c\in \tr_{q^l/q}(C)$. Since $c$ is an arbitrary element in
  $C|_{\F_q}$ it follows that $ C|_{\F_q}\subseteq \tr_{q^l/q}(C)$.
\end{proof}

Let $q=p^s$, then the Euclidean geometry code of order $r$ over
$\eg(m,p^s)$ is defined as the dual of the subfield subcode of
$\Rm_{q}((q-1)(m-r-1),m)$, \cite[page~448]{blahut03}. The type-I LDPC
code $C_{\eg}^{(1)}(m,\mu,0,s,p)$ code is an Euclidean geometry code
of order $\mu-1$ over $\eg(m,p^s)$, see \cite{tang05}\footnote{note
  that there is a small mistake in \cite{tang05} in this respect. The
  authors imply that the $C_{\eg}^{(1)}(m,\mu,0,s,p)$ code is an
  Euclidean geometry code of order $\mu$. It should be $\mu-1$.
  \texttt{[Check again]} }.  Hence its dual is the subfield subcode of
$\Rm_q((q-1)(m-\mu),m)$ code.  In other words,
\begin{eqnarray}
C_{\eg}^{(1)}(m,\mu,0,s,p)^\perp = 
\Rm_q((q-1)(m-\mu),m)|_{\F_p}.\label{eq:fgSubfiledCode}
\end{eqnarray}
Further, Delsarte's theorem \cite{delsarte75} tells us that 
\begin{eqnarray*}
\Rm_q((q-1)(m-\mu),m)|_{\F_p}^\perp &=&\tr_{q/p}\left( \Rm_q((q-1)(m-\mu),m)^\perp\right)\\
&=&  \tr_{q/p}(\Rm_q(\mu(q-1)-1,m)).
\end{eqnarray*}
Hence,  $C_{\eg}^{(1)}(m,\mu,0,s,p)$ code can also be  related to $\Rm_q(\mu(q-1)-1,m)$ as 
\begin{eqnarray}
  C_{\eg}^{(1)}(m,\mu,0,s,p)=\tr_{q/p}(\Rm_q(\mu(q-1)-1),m).\label{eq:fgTraceCode}
\end{eqnarray}

In the following theorem we use all these facts together to construct
a family of asymmetric stabilizer LDPC codes.

\begin{theorem}[Asymmetric EG LDPC Codes]
  Let $p$ be a prime, with $q=p^s$ and $s\geq 1,m\geq 2$. Let $1<
  \mu_z <m$ and $m-\mu_z+1 \leq \mu_x<m$.  Then there exists an
$$
[[p^{ms},k_x+k_z-p^{ms} , d_x/d_z]]_p
$$
asymmetric EG LDPC code, where 
$$k_x=\dim C_{\eg}^{(1)}(m,\mu_x,0,s,p) \mbox{ and }  k_z=\dim C_{\eg}^{(1)}(m,\mu_z,0,s,p);$$
$d_x\geq A_{\eg}(m,\mu_x,\mu_x-1,s,p)+1$ and $d_z\geq A_{\eg}(m,\mu_z,\mu_z-1,s,p)+1$.
\end{theorem}
\begin{proof}
  Let us choose $C_z=C_{\eg}^{(1)}(m,\mu_z,0,s,p)$.  Then from
  equation~(\ref{eq:fgTraceCode}) we have
\begin{eqnarray*}
C_z &=& \tr_{q/p}(\Rm_q(m,\mu_z(q-1)-1)).
\end{eqnarray*}
By Lemma~\ref{lm:inclusion} we know that 
\begin{eqnarray*}
\tr_{q/p}(\Rm_q(\mu_z(q-1)-1),m) &\supseteq&  \Rm_q(\mu_z(q-1)-1,m)|_{\F_p},\\
C_z&\supseteq & \Rm_q((q-1)(m-(m-\mu_z+1)),m)|_{\F_p},
\end{eqnarray*}
where the last inclusion follows from the nesting property of the
generalized Reed-Muller codes. For any order $\mu_x$ such that
$m-\mu_z+1\leq \mu_x <m$, let $C_x=C_{\eg}^{(1)}(m,\mu_x,0,s,p)$. Then
$C_x$ is an LDPC code whose dual $C_x^\perp =
\Rm_q((q-1)(m-\mu_x),m)|_{\F_p}$ is contained in $C_z$. Thus we can
use Lemma~\ref{lm:css} to form an asymmetric code with the parameters
$$ 
[[p^{ms},k_x+k_z-p^{ms} , d_x/d_z]]_p
$$
The distance of $C_z$ and $C_x$ are at lower bounded as 
$d_x \geq A_{\eg}(m,\mu_x,\mu_x-1,s,p)+1$ 
and $d_z \geq A_{\eg}(m,\mu_z,\mu_z-1,s,p)+1$  (see \cite{tang05}).
\end{proof}

In the construction just proposed, we should choose $C_x$ to be a
larger code compared to $C_z$ so that $C_z$ is a stronger code. We
have the construction over a nonbinary alphabet although in the
context of asymmetric quantum codes one might be more interested in
the case $p=2$.

Our final construction is an alternative to the method proposed in
\cite{ioffe07}.  Now we shall make use of the cyclic finite geometry
codes.  Our goal will be to find a small BCH code whose dual is
contained in a cyclic Euclidean geometry LDPC code. For solving this
problem we need to know the cyclic structure of
$C_{\eg,c}^{(1)}(m,\mu,0,s,p)$. Let $\alpha$ be a primitive element in
$\F_{p^{ms}}$. Then the roots of generator polynomial of
$C_{\eg,c}^{(1)}(m,\mu,0,s,p)$ are given by
\cite[Theorem~6]{kasami71}, see also \cite{kasami68b,lin04}.
$$
Z= \{\alpha^h\mid 0< \max_{0\leq l<s} W_{p^s}(h p^l) \leq
(p^s-1)(m-\mu) \},
$$
where $W_{q}(h)$ is the $q$-ary weight of $h = h_0+h_1q+\cdots +
h_kq^{k-1}$ {\em i.e.}  $W_q(h)=\sum h_i$.  The finite geometry code
$C_{\eg,c}^{(1)}(m,\mu,0,s,p)$ is actually an $(\mu-1,p^s)$ Euclidean
geometry code.  The roots of the generator polynomial of the dual code
are given by
$$
Z^{\perp}= \{\alpha^h \mid \min_{0\leq l<s} W_{p^s}(hp^l) < \mu(p^s-1) \}.
$$
In fact, the dual code is the even-like subcode of a primitive
polynomial code of length $p^{ms}-1$ over $\F_p$ and order $m-\mu$,
whose generator polynomial, by \cite[Theorem~6]{kasami68b}, has the
roots
$$
Z_p= \{\alpha^h \mid 0< \min_{0\leq l<s} W_{p^s}(hp^l) < \mu(p^s-1) \}.
$$
Thus $Z^\perp = Z_p\cup \{ 0\}$.  Now by \cite[Theorem~11]{kasami68b},
$Z_p$ and therefore $Z^\perp$ contain the sequence of consecutive
roots, $\alpha,\alpha^2,\ldots, \alpha^{\delta_0-1}$, where
$$\delta_0=(R+1)p^{Qs}-1 \mbox{ and } m(p^s-1)-(m-\mu)(p^s-1) = Q(p^s-1)+R.$$
Simplifying, we see that $R=0$ and $Q=\mu$ giving $\delta_0 = p^{\mu s}-1$.
It follows that 
$$C_{\eg,c}^{(1)}(m,\mu,0,s,p)^\perp = \Rm_q(m,(q-1)(m-\mu))|_{\F_q} \subseteq \bch(\delta_0).$$

Thus we have solved the problem of construction of the asymmetric
stabilizer codes in dual fashion to that of \cite{ioffe07}. Instead of
finding an LDPC code whose parity check matrix is contained in a given
BCH code, we have found a BCH code whose parity check matrix is
contained in a given finite geometry LDPC code. This gives us the
following result.
\begin{lemma}[Asymmetric BCH-LDPC stabilizer codes]
  Let $C=C_{\eg,c}^{(1)}(m,\mu,0,s,p)$ and $\delta\leq \delta_0=p^{\mu
    s}-1$.  Then there exists an
$$[[p^{ms}-1,k_x+k_y-n,d_x/d_z]]_p$$
asymmetric stabilizer code where $d_z\geq A_{\eg}(m,\mu,\mu-1,s,p)$ and
$d_x\geq \delta$. 
\end{lemma}

In what follows we give a small example to illustrate this
construction.

\begin{example}
  \rm Let $m=s=p=2$ and $\mu=1$. Then $C_{\eg,c}^{(1)}(2,1,0,2,2)$ is
  a cyclic code whose generator polynomial has roots given by
\begin{eqnarray*}
  Z&=&\{\alpha^h|0<\max_{0\leq l<2 }W_{2^2}(2^lh) \leq (m-\mu)(p^s-1)=(2-1)(2^2-1) \}\\
  &=&\{  \alpha^1, \alpha^2, \alpha^3, \alpha^4, \alpha^6, \alpha^8, \alpha^9, \alpha^{12} \}.
\end{eqnarray*}
As there are 4 consecutive roots and $|Z|=8$, it defines a $[15,7,\geq
5]$ code.  The roots of the generator polynomial of the dual code are
given by
\begin{eqnarray*}
Z^\perp&=& \{\alpha^h|0<\min_{0\leq l<2 }W_{2^2}(2^lh) \leq \mu(p^s-1)=(2^2-1) \}\\
&=&\{ \alpha^0, \alpha^1, \alpha^2, \alpha^4, \alpha^5, \alpha^8, \alpha^{10} \}.
\end{eqnarray*}
We see that $Z^\perp$ has two consecutive roots excluding $1$,
therefore the dual code is contained in a narrowsense BCH code with
design distance 3. Note that $p^{\mu s}-1=3$.  Thus we can choose
$C_x=\bch(3)$ and $C_z=C_{\eg,c}^{(1)}(2,1,0,2,2)$ and apply
Lemma~\ref{lm:css} to construct a $[[15,3,3/5]]_2$ asymmetric code.
\end{example}

We can also state the above construction in a dual fashion, that is
given a primitive BCH code of design distance $\delta$, find an EG
LDPC code whose dual is contained in it. It must be pointed out that
in case of asymmetric codes derived from LDPC codes, the asymmetry
factor $d_x/d_z$ is not as indicative of the code performance as in
the case of bounded distance decoders.  For $m=p=2$, we can derive
explicit relations for the parameters of the codes.
\begin{corollary}\label{co:2dCyclic}
  Let $C=C_{\eg,c}^{(1)}(2,1,0,s,2)$ and $\delta =2t+1\leq 2^{s}-1$.
  Then there exists an
$$[[2^{2s}-1,2^{2s}-3^s -s(\delta-1),\delta/2^s+1]]_2 $$ 
asymmetric stabilizer code.
\end{corollary}
\begin{proof}
  The parameters of $C$ are $[2^{2s}-1,2^{2s}-3^s,2^{s}+1]_2$, see
  \cite{lin04}. Since $C^\perp $ is contained in a BCH code of length
  $2^{2s}-1$ whose design distance $\delta\leq 2^s-1$, we can compute
  the dimension of the BCH code as $2^{2s}-1 -s(\delta-1)$, see
  \cite[Corollary~8]{macwilliams77}. By Lemma~\ref{lm:css} the quantum
  code has the dimension $2^{2s}-3^s -s(\delta-1)$.
\end{proof}

\begin{example}
  \rm For $m=p=2$ and $s=4$ we can obtain a $[255,175,17]$ LDPC code.
  We can choose any BCH code with design distance $\delta \leq
  2^4-1=15$ to construct an asymmetric code. The following codes are
  possible.  Simulation results are also given for the highlighted
  codes.

\begin{table}[htb]
\begin{center}
\begin{tabular}{c|c|c|l|c}
$s$&$\delta$  & Code &   Asymmetry &Rate\\
&  & $[[n,k,d_x/d_z]]_2$ &    $d_z/d_x$ &\\\hline
4&  15 & $[[255,119,15/17]]_2$   &   $\approx 1$&0.467\\
4&13  & $[[255,127,13/17]]_2 $&  $\approx 1.25$&0.498\\
4&11  & $[[255,135,11/17]]_2 $&  $\approx 1.5$&0.529\\
4&9  & $[[255,143,9/17]]_2 $&  $\approx 2$ &0.561\\
4&7  & $[[255,151,7/17]]_2 $&  $\approx 2.5$&0.592\\
4&5  & $[[255,159,5/17]]_2 $&  $\approx 3$&0.624\\
4&3  & $[[255,167,3/17]]_2 $&  $\approx 6$&0.655\\
\end{tabular}
\end{center}
\caption{Asymmetric quantum codes constructed from the construction 
based on pairs of LDPC and BCH codes.}
\label{tab:bchLdpcAqecc}
\end{table}
\end{example}

\section{Performance Results}
\label{sec:performance}

We now give the performance results of some of the codes constructed
in the previous section.  First we will give the details about the
channel model and how the simulations are performed.

Basically, asymmetric stabilizer codes can give us two benefits. First
of all over an asymmetric quantum channel, they can give lower error
rates compared to symmetric codes. We assume in this case we are
comparing codes of same rates. Secondly, for the same error rates over
asymmetric channels, the asymmetric codes can give higher data rates.
Let us demonstrate these benefits of asymmetric quantum codes by means
of some simple examples. In order to be fair we will compare codes of
similar decoding complexity.

In the simulations we make a simplifying assumption about the channel
model which was first used in \cite{mackay04} to simplify the
simulation quantum LDPC codes.  We assume that the overall probability
of error in the channel is given by $p$, while the individual
probabilities of $X,Y,Z$ errors are $p_x=p/(A+2)$, $p_y=p/(A+2)$ and
$p_z=pA/(A+2)$ respectively. The exact performance would require us to
simulate a $4$-ary channel and also account for the fact that some
errors can be estimated modulo the stabilizer. However, we observed
that if we ignored the effect of the stabilizer it does not change the
error rates because these codes are nondegenerate. The 4-ary channel
can be modeled as two binary symmetric channels one modeling the bit
flip channel and the other the phase flip channel. For exact
performance, these two channels should be dependent, however, a good
approximation is to model the channel as two independent BSCs with
cross over probabilities $p_x+p_y=2p/(A+2)$ and
$p_y+p_z=p(A+1)/(A+2)$. In this case the overall error rate in the
quantum channel is the sum of the error rates in the two BSCs. While
this approach is going to slightly overestimate the error rates,
nonetheless it is useful and commonly used in literature.  Since the
$X$-channel uses a BCH code and decoded using a bounded distance
decoder, we can just compute $P_e^x$ the $X$ error rate, in closed
form as
\begin{eqnarray}
  P_e^x &=&1-\sum_{j=0}^{\floor{(d-1)/2}}
  \binom{n}{j}(p_x+p_y)^j(1-p_x-p_y)^{n-j}.\label{eq:pErrX}
\end{eqnarray}
The error rate in the Z channel, $P_e^z$ is obtained through
simulations. The overall error rate is
$$P_e=1-(1-P_e^x)(1-P_e^z)=P_e^x+P_e^z-P_e^xP_e^z\approx P_e^x+P_e^z.$$ 

\begin{example}[Illustrating improvement of error rate]
  \rm The optimal $[[15,1]]$ code has a distance 5.  It is not
  possible to get a distance higher than 5 for the given $n,k$.
  However, should we use an asymmetric code, then we can get an
  $[[15,1,3/7]]$ code.  This code can be constructed by choosing
  $C_x=\bch(3)$ and $C_z=\bch(7)$ in Lemma~\ref{lm:css}, both of
  length 15.  We now consider the performance of quantum codes over a
  quantum channel of the form
$$\E(\rho) = (1-p) \rho +p_x \X\rho \X +p_y \Y\rho\Y + p_z \Z\rho \Z, 
\mbox{ where } p=p_x+p_y+p_z; p_x=p_y=p_z/A.$$ 
As we vary the channel asymmetry $A=p_z/p_x=p_z/p_y$ we keep the
probability of error $p=p_x+p_y+p_z$ constant.  On a symmetric channel
the asymmetric code is going to fare worse than the symmetric code. If
we increase the asymmetry of the channel then we can see that the code
performance improves. Figure~\ref{fig:exAsymCode1} shows the
performance of $[[15,1,3/7]]$ code over various asymmetric channels.

\begin{figure}[htb]
\begin{center}
%\epsfig{file=n15,scale=0.5}
\epsfig{file=n15dx3dz7varyA,scale=0.6}
\caption{Performance of a $[[15,1,3/7]]$ code described in the text
  for choices $A=1,10,100$ of the channel
  asymmetry.}\label{fig:exAsymCode1}
\end{center}
\end{figure}

While it is not shown here the performance of the symmetric code does
not change too much as the channel asymmetry is varied.  The key
observation is that increasing channel asymmetry improves the
performance of the asymmetric code. Figure~\ref{fig:exAsymCode2}
compares the performance of the symmetric and asymmetric codes.  For
clarity the asymmetric code's performance is shown over three values
of channel asymmetry, while the symmetric code's performance is shown
only when the channel asymmetry is 100, since this is the point of
interest for us.

\begin{figure}[htb]
\begin{center}
\epsfig{file=n15compare,scale=0.6}
\caption{Comparison between the performance of a $[[15,1,3/7]]$ that
  has been described in the text with the performance of a symmetric
  $[[15,1,5]]$. The shown curves are the plots for choices of
  asymmetry parameter $A=1,10,100$ for the asymmetric code and the
  $A=100$ for the symmetric code.}\label{fig:exAsymCode2}
\end{center}
\end{figure}

\end{example}

\begin{example}[Illustrating data rate gain]
  \rm Let us now compare the performance of a $[[31,1,7]]$ quantum BCH
  code with its asymmetric counterpart. There exists a $[[31,11,3/7]]$
  quantum BCH code. In figure~\ref{fig:exAsymCode3}, we see that over
  a channel with asymmetry $A=100$, the performance of the asymmetric
  code is comparable to that of the symmetric code, but we are able to
  operate at a rate 10 times larger.

\begin{figure}[hbt]
\begin{center}
%\epsfig{file=n31,scale=0.5}
\epsfig{file=n31compare,scale=0.6}
\caption{Comparison of the performance of a symmetric $[[31,1,7]]$
  codes and the performance of an asymmetric $[[31,11,3/7]]$ code for
  channel asymmetry $A=100$.}\label{fig:exAsymCode3}
\end{center}
\end{figure}

\end{example}

\paragraph{Decoding LDPC Codes.} The LDPC code was decoded using the
an algorithm similar to the hard decision bit flipping algorithm given
in \cite{kou01}. This is an instance of the bit flipping algorithm
originally given by Gallager.  The maximum number of iterations for
decoding is set to 50. A small modification had to be made to
accommodate the special situation of quantum syndrome decoding. By
measuring the generators of the stabilizer group, we obtain a
classical syndrome, which due to the fact that only $\pm 1$
eigenspaces occur in all of the generators, is hard information. We
use the syndrome as shown in Figure \ref{fig:bp} and initialize all
the bit nodes with $0$ at the start of the algorithm. Then the
algorithm proceeds in the usual fashion as in \cite{kou01}. We
implemented this algorithm and ran several simulations which are
described next.

\begin{figure}[htb]
\begin{center}
\epsfig{file=tanner,scale=1.0} 
\caption{Modification of the iterative message passing algorithm to
  the quantum case. The initialization step is different from the
  classical case as no soft information from the channel is available
  but rather only hard information about the measured syndrome is
  available. The algorithms begins with initializing all bit nodes to
  $0$ and the check nodes with the syndrome. From then on, any
  classically known method for iterative decoding can be applied. In
  the figure this principle is shown for the example of a classical
  [7,4,3] Hamming code. Application to the quantum case is
  straightforward as the decoding algorithm only works with classical
  information to compute the most likely error.}\label{fig:bp}
\end{center}
\end{figure}

In figure~\ref{fig:fg255d7} we see the performance of
$[[255,159,5/17]]$ as the channel asymmetry is varied from 1 to 100.
As we observed with the BCH asymmetric codes in
Section~\ref{sec:performance}, here also we see that as we increase the
asymmetry the code starts to perform better.  As the asymmetry is
increased eventually the performance of the quantum code approaches
the performance of the classical LDPC code. 

\begin{figure}[htb]
\begin{center}
\epsfig{file=n255d5varyAz,scale=0.6} 
\caption{Performance of a $[[255,159,5/17]]$ code described in the
  text for choices $A=1,10,100$ of the channel asymmetry.}\label{fig:fg255d5}
\end{center}
\end{figure}

\begin{figure}
\begin{minipage}[b]{1\linewidth}
\centering
\includegraphics[width=12cm]{n255d7varyAz.eps}
\caption{Performance of a $[[255,151,7/17]]$ code described in the
  text for choices $A=1,10,100$ of the channel asymmetry.}
\label{fig:fg255d7}

\end{minipage}
\hspace{0.5cm} 
\begin{minipage}[b]{1\linewidth}
\centering
\includegraphics[width=12cm]{n255d9varyAz.eps}
\caption{Performance of a $[[255,143,9/17]]$ code described in the
  text for choices $A=1,10,100$ of the channel asymmetry.}\label{fig:fg255d9}
\end{minipage}
\end{figure}

Tolerating a little rate loss improves the performance as can be seen
from figure~\ref{fig:fg255d7}.  If we increase the distance of the BCH
code the code becomes more tolerant to variations in channel asymmetry
as can be seen by the performance of $[[255,143,9/17]]$ in
figure~\ref{fig:fg255d9}.  This plot also illustrates an important
point. Our channel model assumes that as we vary the channel asymmetry
we keep the total probability of error in the channel fixed.  This
implies that while the probability of $X$ errors goes down, the
probability of $Z$ errors tends to $p$, the total probability of
error. Hence, the reduction in error rate in the $X$ channel must more
than compensate for the increase in $Z$ error rate.  If on the other
hand, we had fixed the probability of error in the $Z$ channel and
varied the channel asymmetry then we would observe a monotonic
improvement in the error rate because on one hand the $Z$ error rate
does not change but the $X$ error rate does.

Comparing with the short length codes of Section~\ref{sec:performance}
we see that the error rate falls much more sharply. In fact, with
larger lengths we can get an even steep drop in the error rate as is
apparent from the performances of $[[255,151,7/17]]$ and
$[[1023,731,11/33]]$ code in figures~\ref{fig:n255d7} and
\ref{fig:n1023A100} respectively; both are plotted on the same scale
as the shorter BCH codes of Section~\ref{sec:performance}.

\begin{figure}    
\begin{minipage}[b]{1\linewidth}  
\centering
\includegraphics[width=12cm]{n255d7varyA.eps}
\caption{Performance of  $[[255,151,7/17]]$ code for $A=1,10,100$.}\label{fig:n255d7}
\end{minipage}
\hspace{0.5cm} 
\begin{minipage}[b]{1\linewidth}
\centering
%\includegraphics[width=12cm]{n255d9varyAz.eps}
\epsfig{file=n1023d11A100,scale=0.6}
\caption{Performance of  $[[1023,731,11/33]]$ code for $A=100$.}\label{fig:n1023A100}
\end{minipage}
\end{figure}

\section{Conclusion and discussion}
\label{sec:conclusions}

We have presented several new results regarding asymmetric quantum
error-correcting codes, namely linear programming bounds on the
feasible parameters, constructions based on nested families of
classical codes and a CSS construction based on LDPC/BCH pairs.
Furthermore, we emphasized that for the simulation of these codes a
slight modification of the standard classical belief propagation type
simulation is necessary. We carried out performance simulations for
some asymmetric quantum LDPC codes and found that as expected the
performance is a function of the channel asymmetry. 

The question naturally raises how the codes presented in this work, in
particular those obtained by the LDPC/BCH construction presented in
Section \ref{sec:ldpcbch}, compare with the codes proposed in
\cite{ioffe07}.  Strictly speaking both constructions have regimes
where they can perform better than the other. But it appears that the
algebraically constructed asymmetric codes have the following benefits
with respect to the randomly constructed ones of \cite{ioffe07}.
\begin{itemize}
\item They give comparable performance and higher data rates with
  shorter lengths.
\item The benefits of classical algebraic LDPC codes are inherited
  like low error floors compared to the random LDPC codes.
\item The code construction is systematic.
\end{itemize}
Our codes also offer flexibility in the rate and performance of the
code because we can choose many possible BCH codes for a given finite
geometry LDPC code or vice versa.  The flip side however is that the
codes given here have a slightly higher complexity of decoding.

Open problems are to study the performance of alternatives to the hard
decision bit algorithm used in the performance simulations.
Alternatives would be to study other ways of message passing such as
MLG, weighted bit flipping, APP, belief propagation etc.

Finally, it will be imperative to study whether the codes constructed
in this paper can be used to perform universal fault tolerant quantum
computing on them without changing the bias in the error model.

\section*{Acknowledgment} The authors would like to thank Marcus
Silva for many useful discussions and for proposing the combined
amplitude damping and dephasing channel which is our main motivating
example.  

\bibliographystyle{plain} 
\bibliography{refs} 

\appendices
  
\section{Proof of Theorem 1}
\label{app:theorem1}

\begin{theorem} Given a combined amplitude damping and dephasing
  channel $\mathcal{E}$ as above, the associated Pauli-twirled channel
  is of the form
$$\mathcal{E}_T(\rho) = (1-p_x-p_y-p_z)\rho+ p_x\X\rho\X+p_y\Y\rho\Y +
p_z\Z\rho\Z,$$ where $p_x=p_y=(1-e^{-t/T_1})/4$ and
$p_z=1/2-p_x-\frac{1}{2}e^{-t/T_2}$.  In particular,
$$ \frac{p_z}{p_x} =1+2 \frac{1-e^{t/T_1(1-T_1/T_2)}}{e^{t/T_1}-1}.
$$ 
If $t\ll T_1$, then we can approximate this ratio as $2T_1/T_2-1$.
\end{theorem}

\begin{proof}
  The Kraus operator-sum decomposition of $\mathcal{E}$ is given by
\begin{eqnarray}
\mathcal{E}(\rho) = \sum_{k=0}^2A_k\rho A_k^\dagger,\mbox{ where } 
A_0= \left[\begin{smallmatrix} 1&0
\\0&\sqrt{1-\lambda-\gamma}\end{smallmatrix}\right]; A_1 = \left[\begin{smallmatrix} 0&
0\\0&\sqrt{\lambda}\end{smallmatrix}\right];A_2 = \left[\begin{smallmatrix} 0&
\sqrt{\gamma}\\0& 0\end{smallmatrix}\right],\label{eq:krausDecomp}
\end{eqnarray}
and $\sqrt{1-\gamma-\lambda}= e^{-t/T_2}$, $1-\gamma=e^{-t/T_1}$. We
can rewrite the Kraus operators $A_i$ as
\begin{eqnarray*}
A_0&=&\frac{1+\sqrt{1-\lambda-\gamma}}{2}\one +\frac{1-\sqrt{1-\lambda-\gamma}}{2}\Z,\\
A_1&=&\frac{\sqrt{\lambda}}{2}\one -\frac{\sqrt{\lambda}}{2}\Z,\\
A_2&=&\frac{\sqrt{\gamma}}{2}\X +\frac{\sqrt{\gamma}}{2i}\Y,
\end{eqnarray*}
Rewriting $\E(\rho)$ in terms of Pauli matrices 
yields 
\begin{eqnarray}
  \E(\rho) &=& \frac{2-\gamma+2\sqrt{1-\lambda-\gamma}}{4} \rho + \frac{\gamma}{4}\X\rho\X +\frac{\gamma}{4}\Y\rho\Y +
  \frac{2-\gamma-2\sqrt{1-\lambda-\gamma}}{4}\Z\rho\Z \nonumber \\
  &-& \frac{\gamma}{4}\one\rho\Z -\frac{\gamma}{4}\Z\rho\one -\frac{\gamma}{4i} \X\rho\Y
  +\frac{\gamma}{4i}\Y\rho\X.
\end{eqnarray}
It follows that the Pauli-twirl channel $\mathcal{E}_T$ is of the
claimed form, see~\cite[Lemma 2]{dankert06}.

Computing the ratio $p_z/p_x$ we get
\begin{eqnarray*}
  \frac{p_z}{p_x} &=&\frac{2-\gamma-2\sqrt{1-\lambda-\gamma}}{\gamma} =\frac{1+e^{-t/T_1}-2e^{-t/T_2}}{1-e^{-t/T_1}},\\
  &=&1+2\frac{e^{-t/T_1}-e^{-t/T_2}}{1-e^{-t/T_1}} = 1+2 \frac{1-e^{t/T_1-t/T_2}}{e^{t/T_1}-1} 
  =1+2 \frac{1-e^{t/T_1(1-T_1/T_2)}}{e^{t/T_1}-1}.
\end{eqnarray*}
If $t\ll T_1$, then we can approximate the ratio as $2T_1/T_2-1$, as claimed. 
\end{proof}

\section{Performance of CSS stabilizer codes}
\label{app:CSSperformance}

For the sake of completeness we will review some of the aspects
regarding the performance of quantum codes. We will assume that we
have a Pauli channel of the form
$$
\E(\rho) = (1-p_x-p_y-p_z)\rho+ p_x\X\rho\X+p_y\Y\rho\Y + p_z\Z\rho\Z.
$$
The error rates of a quantum code could be obtained by simulating the
associated additive code over $\F_4$ over a $4$-ary channel with
associated probabilities given by $p_x,p_y,p_z$. One additional aspect
that is not usually highlighted is the fact that the errors in the
stabilizer should not be treated as errors. To get the exact error
rate of the quantum code, this should also be taken into account.  But
ignoring their contribution in simulation of the classical additive
code will give us a conservative picture. In case of pure codes which
are decoded using a bounded distance decoder this will also mean that
the elements of the stabilizer are also unlikely and their
contribution can be ignored.

In the case of the CSS type codes, it is possible to look at the
performance of the codes over two binary symmetric channels instead of
a $4$-ary channel.  In this case the decoding is often simpler and one
can quite often obtain nice bounds on the performance. Once again it
is possible to get the exact performance by simulating the BSCs in a
dependent manner. Alternatively, one could simulate two independent
BSCs and get an upper bound on the performance of the code. We
observed that quite often for small length codes there is not much
difference. The two BSCs can be simulated with crossover probabilities
$p_x+p_y$ and $p_y+p_z$ respectively. This is not equivalent to the
original channel. However, the error rates over this independent BSCs
gives a bound on the performance over the dependent BSCs. For bounded
distance decoders quantum codes this is not too different from the
exact performance. Therefore we are not entirely unjustified in
comparing these instead of the exact performances.

It is necessary to know the performance of the codes we construct. We
can get the exact performance by simulating them using the appropriate
channel. For the depolarizing or in general the Pauli channel we can
get useful bounds on the performance of the quantum code simply by
looking at the performance over the classical binary channels.  Let
$P_{e}(d)$ be the probability of block error using a bounded distance
decoder.
$$
P_{e,}(d,p) = 1 - \sum_{j=0}^{\floor{(d-1}/2}\binom{n}{j}(p)^j(1-p)^{n-j}.
$$
For the case of an $[[n,k,d_x/d_z]]$ CSS code we can get a performance 
bound as follows. 

\begin{eqnarray}
P_{e,CSS} &=& 1-(1-P_e(d_x,p_x+p_y))(1-P_e(d_z,p_y+p_z))\\
&\approx& P_e(d_x,p_x+p_y)+P_e(d_z,p_y+p_z).
\end{eqnarray}

See also \cite{mackay04} where similar arguments are used.

\begin{remark}
  \rm If we are to compare the performance of an $[[n,k,d]]$ non-CSS
  code which is decoded using a bounded distance decoder with a
  $[[n,k,d/d]]$ CSS code which is also decoded using a bounded
  distance decoder, then the CSS code is going to outperform the
  non-CSS code in general. The measure of our performance is the block
  error rate. This is because the CSS code even when it being decoded
  using a bounded distance decoder, it will correct many errors of
  weight greater than $\floor{(d-1)/2}$ unlike the non-CSS code.
\end{remark}

\end{document}

